Reinforcement Learning for Diffusion LLMs with Entropy-Guided Step Selection and Stepwise Advantages

Reinforcement learning (RL) has been effective for post-training autoregressive (AR) language models, but extending these methods to diffusion language models (DLMs) is challenging due to intractable sequence-level likelihoods. Existing approaches therefore rely on surrogate likelihoods or heuristic approximations, which can introduce bias and obscure the sequential structure of denoising. We formulate diffusion-based sequence generation as a finite-horizon Markov decision process over the denoising trajectory and derive an exact, unbiased policy gradient that decomposes over denoising steps and is expressed in terms of intermediate advantages, without requiring explicit evaluation of the sequence likelihood. To obtain a practical and compute-efficient estimator, we (i) select denoising steps for policy updates via an entropy-guided approximation bound, and (ii) estimate intermediate advantages using a one-step denoising reward naturally provided by the diffusion model, avoiding costly multi-step rollouts. Experiments on coding and logical reasoning benchmarks demonstrate state-of-the-art results, with strong competitive performance on mathematical reasoning, outperforming existing RL post-training approaches for DLMs. Code is available at https://github.com/vishnutez/egspo-dllm-rl.

==> NeurIPS2026/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
\item[] Justification: \revision{The abstract and introduction describe three main contributions: (i) a policy gradient for the diffusion MDP that decomposes over denoising steps with stepwise advantages; (ii) tractable estimators using entropy-guided step selection and one-step advantage estimation; and (iii) empirical improvements on coding, logical reasoning, and mathematical reasoning benchmarks. The policy gradient is established in Proposition~\ref{thm:pg_thm} and proved in Appendix~\ref{app:theoretical_results}. The practical algorithms are described in Sections 4.2--4.4 and Algorithm~\ref{alg:epsa}, with the distinction between the exact theoretical gradient and practical approximations clarified at the end of Section 4. Empirical results are reported in Tables~\ref{tab:main_results} and~\ref{tab:coding_results}.}    

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The limitation is included in Appendix \ref{sec:limitation}.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All theoretical results (Proposition~\ref{thm:pg_thm}, Lemma~\ref{lem: error_bound_using_entropy}, and Proposition~\ref{prop:entropy_bound}) are proved in full in Appendix~\ref{app:theoretical_results}, with assumptions explicitly stated in each result and all results numbered and cross-referenced in the main text.

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The algorithm is fully described in Algorithm~\ref{alg:epsa}. Hyperparameters, optimizer settings, LoRA configuration, hardware, batch size, generation length, denoising steps, and task-specific reward functions are all detailed in Appendices \ref{sec:dataset&reward}, \ref{sec:baselines}, \ref{sec:hypsetting}. The base model (LLaDA-8B-Instruct) and all datasets used are publicly available. Code is available at the \href{https://anonymous.4open.science/r/epsa-dllm-rl-5802}{anonymous repo} linked in the abstract.


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Code is available at the \href{https://anonymous.4open.science/r/epsa-dllm-rl-5802}{anonymous repo} linked in the abstract. All datasets used are publicly available.


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All training and evaluation details are provided in Appendix~\ref{sec:hypsetting}, including optimizer (Adam), learning rate, LoRA configuration, batch size, hardware, generation lengths, denoising steps, step budget K, temperature, and checkpoint selection criteria. Reward functions and dataset splits are detailed in Appendix~\ref{sec:dataset&reward}.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not report error bars or confidence intervals. Results are reported as single-run accuracies across multiple generation lengths, following the evaluation protocol of prior work in this area (d1, wd1, SPG, d2), which also do not report error bars.
    

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Appendix~\ref{sec:hypsetting} specifies that training is conducted on 8 NVIDIA H200 GPUs. Training durations are provided per task (4k steps for coding, 6k for mathematical reasoning, 10k for logical reasoning).

    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \revision{The research conforms with the NeurIPS Code of Ethics. The work involves no human subjects or sensitive personal data and evaluates RL post-training methods on reasoning and coding benchmarks.}



\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work presents a foundational RL training algorithm for diffusion language models, evaluated on reasoning and coding benchmarks. It is not tied to any specific application or deployment, and there is no direct path to negative societal impacts beyond those inherent to language model research in general.
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper fine-tunes an existing publicly available model (LLaDA-8B-Instruct) on reasoning tasks and poses no significant misuse risks beyond those of the base model itself.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All datasets and the base model (LLaDA-8B-Instruct) are properly cited with references to their original papers. All assets used are publicly available.
    

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code released in the \href{https://github.com/vishnutez/egspo-dllm-rl}{github repo} documented alongside the paper. Training details, hyperparameters, and implementation specifics are provided in Appendices \ref{sec:dataset&reward}, \ref{sec:baselines}, \ref{sec:hypsetting}, and the algorithm is fully described in Algorithm~\ref{alg:epsa}.
    

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing or research with human subjects.
   
\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing or research with human subjects.
   

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \revision{LLM usage is described in Appendix~\ref{app:llm_usage}.}


\end{enumerate}

==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
\item[] Justification: \revision{The abstract and introduction describe three main contributions: (i) a policy gradient for the diffusion MDP that decomposes over denoising steps with stepwise advantages; (ii) tractable estimators using entropy-guided step selection and one-step advantage estimation; and (iii) empirical improvements on coding, logical reasoning, and mathematical reasoning benchmarks. The policy gradient is established in Proposition~\ref{thm:pg_thm} and proved in Appendix~\ref{app:theoretical_results}. The practical algorithms are described in Sections 4.2--4.4 and Algorithm~\ref{alg:epsa}, with the distinction between the exact theoretical gradient and practical approximations clarified at the end of Section 4. Empirical results are reported in Tables~\ref{tab:main_results} and~\ref{tab:coding_results}.}    

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The limitation is included in Appendix \ref{sec:limitation}.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All theoretical results (Proposition~\ref{thm:pg_thm}, Lemma~\ref{lem: error_bound_using_entropy}, and Proposition~\ref{prop:entropy_bound}) are proved in full in Appendix~\ref{app:theoretical_results}, with assumptions explicitly stated in each result and all results numbered and cross-referenced in the main text.

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The algorithm is fully described in Algorithm~\ref{alg:epsa}. Hyperparameters, optimizer settings, LoRA configuration, hardware, batch size, generation length, denoising steps, and task-specific reward functions are all detailed in Appendices \ref{sec:dataset&reward}, \ref{sec:baselines}, \ref{sec:hypsetting}. The base model (LLaDA-8B-Instruct) and all datasets used are publicly available. Code is available at the \href{https://anonymous.4open.science/r/epsa-dllm-rl-5802}{anonymous repo} linked in the abstract.


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Code is available at the \href{https://anonymous.4open.science/r/epsa-dllm-rl-5802}{anonymous repo} linked in the abstract. All datasets used are publicly available.


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All training and evaluation details are provided in Appendix~\ref{sec:hypsetting}, including optimizer (Adam), learning rate, LoRA configuration, batch size, hardware, generation lengths, denoising steps, step budget K, temperature, and checkpoint selection criteria. Reward functions and dataset splits are detailed in Appendix~\ref{sec:dataset&reward}.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not report error bars or confidence intervals. Results are reported as single-run accuracies across multiple generation lengths, following the evaluation protocol of prior work in this area (d1, wd1, SPG, d2), which also do not report error bars.
    

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Appendix~\ref{sec:hypsetting} specifies that training is conducted on 8 NVIDIA H200 GPUs. Training durations are provided per task (4k steps for coding, 6k for mathematical reasoning, 10k for logical reasoning).

    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \revision{The research conforms with the NeurIPS Code of Ethics. The work involves no human subjects or sensitive personal data and evaluates RL post-training methods on reasoning and coding benchmarks.}



\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work presents a foundational RL training algorithm for diffusion language models, evaluated on reasoning and coding benchmarks. It is not tied to any specific application or deployment, and there is no direct path to negative societal impacts beyond those inherent to language model research in general.
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper fine-tunes an existing publicly available model (LLaDA-8B-Instruct) on reasoning tasks and poses no significant misuse risks beyond those of the base model itself.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All datasets and the base model (LLaDA-8B-Instruct) are properly cited with references to their original papers. All assets used are publicly available.
    

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code released in the \href{https://github.com/vishnutez/egspo-dllm-rl}{github repo} documented alongside the paper. Training details, hyperparameters, and implementation specifics are provided in Appendices \ref{sec:dataset&reward}, \ref{sec:baselines}, \ref{sec:hypsetting}, and the algorithm is fully described in Algorithm~\ref{alg:epsa}.
    

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing or research with human subjects.
   
\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing or research with human subjects.
   

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \revision{LLM usage is described in Appendix~\ref{app:llm_usage}.}


\end{enumerate}

==> plots/bar_plot_sudoku.tex <==
% --- clean bar plot, full control over spacing ---
\begin{figure}[ht]
\centering
\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width=25pt,      % <-- bar width
    width=0.5\textwidth,
    height=5cm,
    ylabel={Accuracy (\%)},
    ymin=0, ymax=100,
    ytick={0,25,50,75,100},
    xtick={},
    axis x line*=bottom,    % <-- remove x-axis and ticks
    axis y line*=left,
    % enlarge x limits=4,
    nodes near coords,
    every node near coord/.append style={
        font=\small,
        /pgf/number format/fixed,
        /pgf/number format/precision=1
    },
]

% x positions explicitly control bar centers
\addplot[draw=none, fill=icmlgray]   coordinates {(0,11.8)};
\addplot[draw=none, fill=icmlblue30] coordinates {(1,22.1)};
\addplot[draw=none, fill=icmlblue50] coordinates {(2,25.2)};
\addplot[draw=none, fill=icmlblue70] coordinates {(3,91.9)};
\addplot[draw=none, fill=icmlred]    coordinates {(4,92.8)};

\end{axis}
\end{tikzpicture}
\caption{Sudoku 
enchmark results comparing various models.}
\end{figure}

